From Bugs to Benefits: Improving User Stories by Leveraging Crowd Knowledge with CrUISE-AC

Costs for resolving software defects increase exponentially in late stages. Incomplete or ambiguous requirements are one of the biggest sources for defects, since stakeholders might not be able to communicate their needs or fail to share their domain specific knowledge. Combined with insufficient developer experience, teams are prone to constructing incorrect or incomplete features. To prevent this, requirements engineering has to explore knowledge sources beyond stakeholder interviews. Publicly accessible issue trackers for systems within the same application domain hold essential information on identified weaknesses, edge cases, and potential error sources, all documented by actual users. Our research aims at (1) identifying, and (2) leveraging such issues to improve an agile requirements artifact known as a "user story". We present CrUISE-AC (Crowd and User Informed Suggestion Engine for Acceptance Criteria) as a fully automated method that investigates issues and generates non-trivial additional acceptance criteria for a given user story by employing NLP techniques and an ensemble of LLMs. CrUISE- AC was evaluated by five independent experts in two distinct business domains. Our findings suggest that issue trackers hold valuable information pertinent to requirements engineering. Our evaluation shows that 80-82% of the generated acceptance criteria add relevant requirements to the user stories. Limitations are the dependence on accessible input issues and the fact that we do not check generated criteria for being conflict-free or non-overlapping with criteria from other user stories.

==> commands.tex <==
\makeatletter
\newcounter{todofootnote}
\renewcommand{\@todo}[2][]{%
  \if@todonotes@prependcaptionglobal%
    \@todonotes@prependcaptiontrue%
  \else%
    \@todonotes@prependcaptionfalse%
  \fi%
  \renewcommand{\@todonotes@text}{#2}%
  \renewcommand{\@todonotes@caption}{#2}%
  \setkeys{todonotes}{#1}%
  \if@todonotes@localdisable%
    \else%
        \addtocounter{@todonotes@numberoftodonotes}{1}%
    \if@todonotes@appendtolistoftodos%
        \phantomsection%
        \if@todonotes@captiongiven%
            \else%
            \renewcommand{\@todonotes@caption}{#2}%
        \fi%
        \@todonotes@addElementToListOfTodos%
    \fi%
    % Prepend the short caption given if it is requested
    \if@todonotes@captiongiven%
        \if@todonotes@prependcaption%
            \renewcommand{\@todonotes@text}{\@todonotes@caption: #2}%
        \fi%
    \fi%
    % Place the todonote as indicated by the options (inline or in a
    % marginpar), below is the code for the inline placement.
    % was: \@todonotes@drawMarginNoteWithLine%
    \let\oldthefootnote\thefootnote%
    \renewcommand{\thefootnote}{\roman{footnote}}%
    \footnote[\value{@todonotes@numberoftodonotes}]{\textcolor{red}{TODO: #2}}%
    \let\thefootnote\oldthefootnote%
  \fi%    
}%
\makeatother

\lstnewenvironment{pythoncode}[1][]
  {\lstset{
      language=Python,
      basicstyle=\ttfamily,
      keywordstyle=\color{blue},
      commentstyle=\color{green},
      stringstyle=\color{red},
      numbers=left,
      numberstyle=\tiny,
      stepnumber=1,
      frame=single,
      breaklines=true,
      showstringspaces=false,
      #1
  }}
  {}

\newcommand\todobox[1]{    
    \colorbox{yellow!30}{\textbf{TODO} #1}                
}  

% comments by author
\newcommand{\thomas}[1]{\todo{[TS]: #1}}
\newcommand{\oldthomas}[1]{}
\newcommand{\stefan}[1]{\todo{[SS]: #1}}
\newcommand{\oldstefan}[1]{}

\newenvironment{nospaceflalign*}
 {\setlength{\abovedisplayskip}{0pt}\setlength{\belowdisplayskip}{10pt}%
  \csname flalign*\endcsname}
 {\csname endflalign*\endcsname\ignorespacesafterend}

 \newcommand\iamhere{    
    \colorbox{red!30}{\textbf{--- I am here ---}\hfill}
}  

\newtcbox{\redbox}{
  on line, 
  boxrule=1pt, 
  boxsep=0pt, 
  top=1pt,
  left=1pt, 
  bottom=1pt, 
  right=1pt, 
  colback=white,
  colframe=red,  
  sharp corners}

% algorithm
\algnewcommand{\LeftComment}[1]{\Statex {// #1 }}
\algnewcommand{\RightComment}[1]{// #1}
\makeatletter
\algnewcommand{\LineComment}[1]{\Statex \hskip\ALG@thistlm {// #1}}
\makeatother

\newtoggle{peerreview}

% for figures
\newcommand{\horizontalsep}{2}
\newcommand{\verticalsep}{0.3}
\newcommand{\oversep}{0.3}
\newcommand{\archeight}{0.5}

\newcommand{\draft}[1]{\textcolor{blue}{#1}}

==> sections/approach/prompt_eval_ac.tex <==
\begin{figure}[htb]
    \begin{tcolorbox}[boxsep=0mm, left=2mm]
        \begin{small}
            \begin{flushleft}            
                For the following userstory listed under {[User Story]} and the supplied existing acceptance 
                criteria listed under {[Acceptance Criteria]} tell me, if the new acceptance criteria listed 
                as {[New Acceptance Criteria]} adds any unique, novel or surprising insights and cannot be 
                considered as common knowledge. Your response LABEL must be either ``relevant'' or ``irrelevant''. 
                ``relevant'' means, {[New Acceptance Criteria]} adds valuable and not common knowledge. Here is the data:
                \\[0.5em]
                {[BEGIN DATA]}\\
                ************\\[-0.25em]
                {[User Story]}\\            
                \textcolor{blue}{\textit{\textless insert user story\textgreater}}\\
                ************\\[-0.25em]
                {[Acceptance Criteria]}\\
                \textcolor{blue}{\textit{\textless insert list of existing acceptance criteria\textgreater}}\\
                ************\\[-0.25em]
                {[New Acceptance Criteria]}\\
                \textcolor{blue}{\textit{\textless insert newly generated acceptance criteria\textgreater}}\\  
                ************\\[-0.25em]
                {[END DATA]}
                \\[0.5em]
                Your response should include the LABEL along with an EXPLANATION.
                \\[0.5em]
                Example response:\\
                ************\\[-0.25em]
                LABEL: ``relevant'' or ``irrelevant''\\
                EXPLANATION: An explanation of your reasoning for why the {[New Acceptance Criteria]} adds relevant information to the [User Story].\\
                ************
            \end{flushleft}
        \end{small}
    \end{tcolorbox}        
    \caption{Prompt to assess the usefulness of an acceptance criteria}
    \label{prompt_evaluate}
\end{figure}

==> sections/approach/prompt_gen_ac.tex <==
\begin{figure}[ht]
    \begin{tcolorbox}[boxsep=0mm, left=2mm]
        \begin{small}
            \begin{flushleft}
                Use the following issue listed under {[Issue]} to generate one new acceptance criterion in gherkin format (GIVEN-WHEN-THEN) for the user story in {[User Story]}.                
                \\[0.5em]                
                {[BEGIN DATA]}\\        
                ************\\[-0.25em]
                {[Issue]}\\
                \textcolor{blue}{\textit{\textless insert issue\textgreater}}\\
                ************\\[-0.25em]
                {[User Story]}\\
                \textcolor{blue}{\textit{\textless insert user story\textgreater}}\\
                ************\\[-0.25em] 
                {[END DATA]}
            \end{flushleft}
        \end{small}        
    \end{tcolorbox}    
    \caption{Prompt to generate Gherkin-style acceptance criteria from an issue}
    \label{prompt_generate}
\end{figure}

==> sections/evaluation/evaluation.tex <==
\subsection{Data Sources}

\input{sections/evaluation/issues.tex}
\input{sections/evaluation/userstories.tex}

\subsection{Evaluation Procedure}
We evaluated our approach described in Section~\ref{sec:approach} for all 307 user 
stories.
Every user story had to pass CrUISE-score as outlined in Section~\ref{sec:classification} 
first, resulting in the class assignments displayed in Table~\ref{table_stories_by_class}.

If the determined class was 0 or 1, the process did not continue for the specific user story. 
This either meant, the user story contained syntactical errors according to AQUSA\cite{Lucassen2016aqusa} 
or the role-specific issue corpus $I^{TR}$ as outlined in Section~\ref{sec:role_extraction} was 
not expected to yield good matches. Thus, 175 user stories were skipped.

\begin{table}[htb]    
    \let\TPToverlap=\TPTrlap
    \centering
    \begin{comment}
        use github_20240706
        select count(*), MetricScore from UserStories
        where userstories.ProjectID in (13,14,18)
            and Relevant = 1
        group by MetricScore
    \end{comment}
    \caption{User stories by CrUISE-score}
    \label{table_stories_by_class}
    %\vspace{-1em} % Adjust this value as needed
    \begin{threeparttable}    
        \centering        
        \begin{tabular}{c|c|c}
            \hline
            \bfseries Class & \bfseries \# US & \bfseries Ratio \\
            \hline
            0   & 129 & 42\%\\
            1	& 46 & 15\%\\
            2   & 87 & 28\%\\        
            3	& 24 & 8\%\\ 
            4   & 21 & 7\%\\ % double-checked and confirmed
            \hline
            Total   & 307 & 100\%\\
            \hline
        \end{tabular}           
    \end{threeparttable}   
\end{table}       

132 user stories that CrUISE-score placed into higher classes were processed further. 
Acceptance criteria were generated for all user stories within these classes, 
excluding 6 as they where placed into outlier clusters by DBSCAN. 
Fig.~\ref{fig:stories_by_cluster_size} presents the number of user stories by cluster sizes.

\begin{figure}[htb]
    \centering
    %\resizebox{!}{6cm}{    
        \begin{tikzpicture}
            \begin{axis}[
                ybar,
                symbolic x coords={1,2,3,4,5,6,7},
                xtick=data,
                xticklabel style={align=center, font=\footnotesize},
                xticklabels={
                    $<10$, $<20$, $<40$, $<60$, $<100$, $<150$, $\geq150$
                },
                ylabel={Number of User Stories},
                xlabel={Cluster Size},
                ymin=0,
                ymax=35,
                bar width=15pt,
                nodes near coords,
                height=5cm,
                width=0.46\textwidth
            ]
            \addplot coordinates {(1,20) (2,20) (3,20) (4,17) (5,16) (6,6) (7,27)};
            \end{axis}
        \end{tikzpicture}
    %}
    \vspace{0.5em}
    \caption{Number of User Stories by Cluster Size}
    \label{fig:stories_by_cluster_size}
\end{figure}

The average cluster size was 131. We took random issue samples from each cluster to 
automatically generate and evaluate acceptance criteria until we had a maximum of 
10 relevant criteria for every user story.

\begin{comment}
Algorithm \ref{algorithm_generate} outlines the generation and assessment procedure. 
The maximum number of relevant acceptance criteria, denoted as $max\_ac$, was set to 
10 (Line 1, Line 9). Issues within cluster $C_1$ were selected randomly (Line 3). 
Generation and assessment were performed if the current item was not the user story itself (Line 5).
The function call \textsc{Generate} in Line 6 refers to the prompt presented in 
Section~\ref{ac_generation}. \textsc{Assess} in Line 7 makes use of the prompt in 
Section~\ref{sec:assessment}.

\begin{algorithm}[!htp]
    \caption{Generate and assess acceptance criteria}\label{algorithm_generate}
    \begin{algorithmic}[1]       
        \State $max\_ac = 10$
        \State $relevant\_count = 0$
        \State $C_1^S = \textsc{Shuffle}(C_1)$ \RightComment{randomize cluster}
        \ForAll{$i \in C_1^S$}
            \If{$i \neq U_1^T$} \RightComment{if $i$ is not the user story itself}
                \State $ac = \textsc{Generate}(i)$
                \State $is\_relevant = \textsc{Assess}(ac)$
                \State \textbf{if} $is\_relevant$ \textbf{then} $relevant\_count+= 1$                
                \State \textbf{if} $relevant\_count == 10$ \textbf{then break} 
            \EndIf
        \EndFor
    \end{algorithmic}
\end{algorithm}
\end{comment}

All generated acceptance criteria being assessed as ``relevant''  were inspected manually by 
an eCommerce expert having accumulated more than 20 years of project experience in the eCommerce 
sector, including 8 years agile project management. 
% Furthermore, he has worked as a project 
% manager and requirements engineer for more than 50 medium to large web projects, with the 
% majority concentrated in the book industry. 
A total of 1,094 acceptance criteria were produced automatically. The results were manually 
evaluated to determine whether they constituted a valid addition to the business scope of the 
user story, described edge cases, or covered other non-obvious scenarios.
Acceptance criteria that met the aforementioned conditions were tagged as ``relevance approved''.

The manual inspection of results conducted solely by one expert may pose 
a threat to the validity of this study's outcomes. A more robust approach involves parallel 
inspection by multiple domain experts, determining an appropriate agreement rate, such as 
Cohen's kappa \cite{mchugh2012interrater}, and basing approval on this rate. This will be 
addressed in future research as outlined in Section~\ref{future_research}.

==> sections/evaluation/ratio_figure.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            ybar,
            bar width=0.5cm,
            enlargelimits=0.2,
            ylabel={Avg. number of acceptance criteria},
            xlabel={CrUISE-score class},
            symbolic x coords={2, 3, 4},
            xtick=data,
            nodes near coords,
            every node near coord/.append style={font=\small},
            legend style={at={(0.03,0.98)},anchor=north west}            
        ]
            % not relevant AC
            \addplot+[
                ybar
            ] coordinates {
                (2, 6.26)
                (3, 3.37)
                (4, 1.38)
            }; 
            
            % relevant AC
            \addplot+[
                ybar
            ] coordinates {
                (2, 1.74)
                (3, 4.63)                
                (4, 7.62)
            };
        
            \legend{Irrelevant, Relevant}
            \end{axis}
    \end{tikzpicture}
    \caption{Comparison of irrelevant and relevant acceptance criteria}
    \label{fig:stacked_bar_chart}
\end{figure}

==> sections/evaluation/results.tex <==
\subsection{Results}\label{sec:results}
We applied CrUISE-AC to 132 user stories that fell in the CrUISE-score classes 2, 3, and 4.
The automatic assessment of generated acceptance criteria as outlined in 
Section~\ref{sec:assessment} determined on average 8.5 criteria as relevant 
for a given user story $U_1$. These criteria were manually reviewed and the 
decision was either approved or declined. Table~\ref{tab:avg_relevant_ac} shows, 
for each CrUISE-score class, the average number of acceptance criteria identified 
as relevant by GPT-4 Turbo, those manually approved, and their corresponding ratio. 
For the highest CrUISE-score class 4, manual approval rate was 85\% followed by class 3 with 58\%.

\begin{table}[htb]
    \let\TPToverlap=\TPTrlap
    \centering    
    \begin{comment}
        use github_20240706
        select MetricScore, avg(cast(TotalRelevant as float)) as [Avg Relevant], avg(Total) as [Avg Total]
        from
        (
            select distinct UserStories.ID, UserStories.MetricScore,        
                (select count(*) 
                from UserStories_Gen_AC_final ac
                where ac.StoryID = UserStories.ID                    
                    and ac.RelevantManual = 1            
                ) as [TotalRelevant],
                (select count(*) 
                from UserStories_Gen_AC_final ac
                where ac.StoryID = UserStories.ID

                    and ac.Relevant = 1       
                ) as [Total]
            from UserStories
            join UserStories_Gen_AC_final on UserStories_Gen_AC_final.StoryID = userstories.ID
        ) p
        group by p.MetricScore
    \end{comment}
    \caption{Ratio between relevant and approved AC}
    \label{tab:avg_relevant_ac}    
    \begin{threeparttable}        
        \begin{tabular}{@{}p{0.485\textwidth}@{}}
            \centering
            \begin{tabular}{c|c|c|c}
                \hline
                \bfseries Class & \bfseries Relevant\tnote{1} & \bfseries Approved\tnote{2} & \bfseries Ratio\\
                \hline
                2 & 8 & 1.74 & 22\%\\
                3 & 8 & 4.63 & 58\%\\
                4 & 9 & 7.62 & 85\%\\
                \hline
            \end{tabular}   
        \end{tabular}   
        \begin{tablenotes}[flushleft]\footnotesize 
            \item[1] Number of acceptance criteria assessed as relevant by GPT-4 Turbo               
            \item[2] Number of relevant acceptance criteria approved by manual inspection
        \end{tablenotes}
    \end{threeparttable}    
\end{table}\oldthomas{Wouldn't it make more sense to give absolute numbers here instead of averages?}

For user stories in CrUISE-score classes 2, 3, and 4, Table~\ref{tab:relevant_ac} shows 
the number of stories where relevant and manually approved acceptance criteria were added. 
In the highest class (Class 4), 95\% of user stories were augmented with additional 
valuable acceptance criteria, while 70\% of user stories in Class 3 received similar enhancements.
Unfortunately, the ratio of user stories in class 4 is quite low ($\sim$7\%). However, having 
a fully automated approach that enhances 7\% of user stories with a very high probability (not 
wasting people's time by huge amounts of irrelevant information) is already offering a valuable 
improvement to the state-of-the-art. Moreover, another 8\% of user stories (Class 3) can be improved 
with a moderate probability and, hence, more manual effort to assess the relevance of generated 
criteria. In addition to that, our approach yields hints to improve user stories when they are not 
in the highest class, such that more stories could benefit from our approach when these hints are applied.

\begin{table}[htb]
    \let\TPToverlap=\TPTrlap
    \centering
    \begin{comment}
        use github_20240706
        select UserStories.MetricScore, 
            count(distinct UserStories.ID) AS [Relevant],
            (select count(*) as [Count]
            from UserStories u2
            where u2.ID in (
                    select distinct StoryID 
                    from UserStories_Gen_AC_final
                    where 
                        u2.ProjectID in (13,14,18) 
                        and u2.Relevant = 1                        
                        and u2.MetricScore = UserStories.MetricScore
            )) + 
            (select count(*) 
            from UserStories u2 
            join UserStories_Results r on u2.ID = r.ID
            where r.SizeCluster = -1 and u2.MetricScore = UserStories.[MetricScore]
                and u2.ProjectID in (13,14,18) 
                and u2.Relevant = 1                        
            ) as [Total]
        from UserStories
        join UserStories_Gen_AC_final on UserStories_Gen_AC_final.StoryID = userstories.ID
        where 
            Userstories.ProjectID in (13,14,18)
            and UserStories.Relevant = 1    
            and UserStories_Gen_AC_final.RelevantManual = 1    
        group by UserStories.MetricScore
    \end{comment}        
    \caption{Number of user stories with relevant AC}
    \label{tab:relevant_ac}
    \begin{threeparttable}
        \begin{tabular}{@{}p{0.485\textwidth}@{}}
            \centering
            \begin{tabular}{c|c|c|c}
                \hline
                \bfseries Class & \bfseries Total\tnote{1} & \bfseries Relevant\tnote{2} & \bfseries Ratio\\
                \hline
                2 & 87 & 43 & 49\%\\
                3 & 24 & 17 & 70\%\\
                4 & 21 & 20 & 95\%\\
                \hline
            \end{tabular}   
        \end{tabular}   
        \begin{tablenotes}[flushleft]\footnotesize 
            \item[1] Number of stories in this class
            \item[2] Number of stories with manually approved acceptance criteria                
        \end{tablenotes}
    \end{threeparttable}
\end{table}
     
A complete example of a user story, its existing acceptance criteria along with a newly 
generated and manually approved criteria is displayed in Fig.~\ref{story_1}.
We provide the complete results available for 
access.\footnote{\iftoggle{peerreview}{Supplementary material: generated\_acceptance\_criteria.xlsx}{\url{https://zenodo.org/records/12819736}}}

\input{sections/evaluation/story_1.tex}


==> sections/evaluation/story_1.tex <==
\begin{figure}[htb]
    \begin{tcolorbox}[colback=white, boxsep=0mm, left=2mm]    
        \begin{small}
            \begin{flushleft}
                \textbf{User story}\\
                As a user, I would like to delete an item in the shopping basket in order to remove it from the shopping basket.\\            
            \end{flushleft}
            \begin{flushleft}
            \textbf{Original acceptance criteria}
                \begin{itemize}[leftmargin=0.3cm]
                    \item[--] One ``Remove item'' button is displayed for each item 
                    \item[--] Click on ``Delete'' to remove the item from the shopping cart                
                \end{itemize}  
            \end{flushleft}  
            \begin{flushleft}        
                \textbf{Newly generated and suggested Acceptance Criteria}\\
                Scenario: Free shipping method should disappear when the order amount falls below the free shipping threshold after removing an item\\
                \begin{itemize}
                    \setlength{\itemindent}{-0.5cm}
                    \item[] GIVEN I have items in my shopping basket eligible for free shipping
                    \item[] WHEN I remove one or more items causing the total amount to fall below the free shipping threshold
                    \item[] THEN the free shipping method should no longer be available in the checkout options.
                \end{itemize}
            \end{flushleft}
        \end{small}
    \end{tcolorbox}    
    \caption{User story enriched with new acceptance criteria}
    \label{story_1}
\end{figure}

==> sections/evaluation/userstories.tex <==
\subsubsection{User Stories}
For this study, user stories from three distinct industry-specific closed-source projects were accessible.
All projects are related to e-commerce, specifically targeting the book industry in German-speaking countries. 
The projects were managed by different product owners, therefore user stories were written by different authors.

\begin{itemize}[leftmargin=0.25cm]    
    \setlength{\itemindent}{-0.25cm}
    % Stollfuss
    \item[] \textbf{Project A} defines a complete set of requirements for a B2C focused online shop 
            of a publishing house who aims to sell its own publications directly.
    % MANZ
    \item[] \textbf{Project B} contains a partial set of requirements for a B2C focused online shop of a bookseller. 
    % Sack
    \item[] \textbf{Project C} includes a subset of B2C and B2B requirements for an online bookstore, 
            supplemented by an e-procurement module designed to provide information and automation for industrial customers.
\end{itemize}

Since acceptance criteria are optional, not all user stories came with them. 
Table~\ref{table_userstories} presents the number of user stories (US) we received by project along with the 
individual distribution between user stories with and without additional acceptance criteria (AC). 
We provide the dataset for access and 
review.\footnote{\iftoggle{peerreview}{Supplementary material: User stories.xlsx}{\url{https://zenodo.org/records/12754330}}}

\begin{table}[htb]    
    \let\TPToverlap=\TPTrlap
    \centering
    \begin{comment}
        use github_20240706
        select count(*), Projects.Name
        from UserStories 
        join Projects on UserStories.ProjectID = projects.ID
        where Relevant = 1
            and ProjectID in (13,14,18)
            and AcceptanceCriteriaCombined is not null
        group by Projects.Name

        select count(*), ProjectID
        from UserStories 
        where Relevant = 1
            and ProjectID in (13,14,18)
            and AcceptanceCriteriaCombined is not null
        group by ProjectID
    \end{comment}
    \caption{User Stories by Project}
    \label{table_userstories}            
    \begin{threeparttable}
        \begin{tabular}{@{}p{0.485\textwidth}@{}}
            \centering        
            \begin{tabular}{c|c|c|c}
                \hline
                \bfseries Project & \bfseries \# US & \bfseries with AC & \bfseries Ratio \\
                \hline
                Project A   & 127 & 87 & 69\% \\
                Project B	& 112 & 112 & 100\% \\
                Project C	& 40 & 14 & 35\%\\
                \hline
                Total       & 307 & 213 & 69\%\\
                \hline
            \end{tabular}   
        \end{tabular}   
    \end{threeparttable}    
\end{table}    

\begin{comment}
    select lang, Projects.Name, count(*) from UserStories 
    join Projects on UserStories.ProjectID = projects.ID
    where ProjectID in (13,14,18) and Relevant = 1
    group by lang, Projects.Name
\end{comment}
250 out of 307 user stories along with their acceptance criteria were written in German language. 
To match them against the collected issues written in English, user stories in German had to be translated. 
For this purpose, we used the API provided by DeepL\cite{deepl2024}.
\oldthomas{Why 250? How many of the translated US had AC? Could the table be extended accordingly? --> Stefan: resolved}

All user stories and acceptance criteria were anonymized. Company names were 
replaced by neutral terms such as ``merchant'' or ``shop owner'', contained URLs were removed.
